Advantages of Bilinear Koopman Realizations for the Modeling and Control of Systems with Unknown Dynamics

Nonlinear dynamical systems can be made easier to control by lifting them into the space of observable functions, where their evolution is described by the linear Koopman operator. This paper describes how the Koopman operator can be used to generate approximate linear, bilinear, and nonlinear model realizations from data, and argues in favor of bilinear realizations for characterizing systems with unknown dynamics. Necessary and sufficient conditions for a dynamical system to have a valid linear or bilinear realization over a given set of observable functions are presented and used to show that every control-affine system admits an infinite-dimensional bilinear realization, but does not necessarily admit a linear one. Therefore, approximate bilinear realizations constructed from generic sets of basis functions tend to improve as the number of basis functions increases, whereas approximate linear realizations may not. To demonstrate the advantages of bilinear Koopman realizations for control, a linear, bilinear, and nonlinear Koopman model realization of a simulated robot arm are constructed from data. In a trajectory following task, the bilinear realization exceeds the prediction accuracy of the linear realization and the computational efficiency of the nonlinear realization when incorporated into a model predictive control framework.

==> unused/0_abstract_old.tex <==
% %% Global linear embeddings of nonlinear systems have enabled control
% The Koopman operator provides a global linear embedding of nonlinear dynamical systems in the (infinite-dimensional) space of real valued functions, called observables.
% % which enables them to be controlled using computationally efficient techniques.
% Such --- are linear with respect to the observables, but not necessarily the contro input
% %% But, not all controlled dynamical systems have a linear embedding, even in infinte dimensions
%
% Global linear embeddings of nonlinear controlled dynamical systems enables them to be controlled using computationally efficient techniques.
% The Koopman operator provides such a linear embedding in the space of all real-valued functions, called observables.
%
% Nonlinear systems can be made easier to control by converting them into equivalent linear or bilinear realizations in the space of real-valued functions, called observables \Dan{Use better words in this sentence, could use help!}.
Nonlinear dynamical systems can be made easier to control by lifting them into the space of observable functions, where their evolution is described by the linear Koopman operator.
%
In this paper, we describe how the Koopman operator can be used to generate linear, bilinear, and nonlinear model realizations
% that are compatible with computationally efficient control methods.
%
and we present necessary and sufficient conditions for a nonlinear dynamical system to have a linear or bilinear realization in the subspace spanned by a given set of observables.
%
We show that every control-affine system admits a valid bilinear realization over an infinite-set of observables, but does not necessarily admit a linear one.
%
Given this result, we argue that when the dynamics of a system are unknown, a bilinear Koopman realization constructed from data is likely to yield better prediction and control results that a linear or nonlinear Koopman realization.
%
% Given this result, we argue that for system identification and control of systems with unknown dynamics, bilinear Koopman realizations are the best choice.
%
To justify this claim, we construct several linear, bilinear, and nonlinear Koopman realizations of a simulated robot arm from data.
%
Using this example we demonstrate how a bilinear Koopman realization simultaneously exceeds the prediction accuracy of a linear Koopman realization and the computational efficiency of a nonlinear Koopman realization.


% To justify this claim, we present a method for constructing linear, bilinear, and nonlinear Koopman realizations from data.
% %
% Then, using a simulated robot arm, we demonstrate how a bilinear Koopman realization simultaneously exceeds the prediction accuracy of a linear Koopman realization and the computational efficiency of a nonlinear Koopman realization.


==> unused/2_theory_old.tex <==
\section{Theory}    \label{sec:theory}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Koopman operator preliminaries
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Koopman operator preliminaries}  \label{sec:preliminaries}

\Dan{Can edit/shorten first few paragraphs to be more concise and not self-plagiarize.}
Consider the (nonlinear) dynamical system governed by the following differential equation
\begin{align}
    \dot{\xvec}(t) &= \Fvec ( \xvec(t) , \uvec(t) )
    % \dot{\xvec}(t) &= \Fvec_x (\xvec(t)) + \Fvec_{xu} ( \xvec(t) , \uvec(t) )
    % y(t) &= g( x(t) )
    \label{eq:nlsys}
\end{align}
where $\xvec(t) \in X \subset \Real^n$ is the output and $\uvec(t) \in U \subset \Real^m$ is the input of the system at time $t \in [0 , +\infty)$, $\Fvec_x, \Fvec_{xu}$ are continuously differentiable functions, and $X, U$ are compact subsets.
Denote by $\phi_\tau : X \times U \to X \times U$ the \emph{flow map}, where $\phi_\tau ( \xvec(0) , \uvec(0) ) = ( \xvec(\tau) , \uvec(0) )$ and $\xvec(\tau)$ is the solution to \eqref{eq:nlsys} at time $\tau$ when beginning with the initial condition $\xvec(0)$ at time $0$ and a constant input $\uvec(0)$ applied for all time between $0$ and $\tau$.

%% System representation in the space of observables
The system can be lifted to an infinite-dimensional function space $\mathcal{F}$ composed of all square-integrable real-valued functions with compact domain $X \times U \subset \Real^{n \times m}$.
Elements of $\mathcal{F}$ are called \emph{observables}.
In $\mathcal{F}$, the flow of the system is characterized by the set of Koopman operators $\koop_\tau : \mathcal{F} \to \mathcal{F}$, for each $\tau \geq 0$,
which describe the evolution of the observables ${f \in \mathcal{F}}$ along the trajectories of the system according to the following definition:
\begin{align}
    \koop_\tau f = f \circ \phi_\tau,      
    \label{eq:koopman}
\end{align}
where $\circ$ indicates function composition such that
\begin{align}
    ( \koop_\tau  f) (\xvec(t),\ucon ) 
    % &= f \left( \phi_\tau( \xvec(t),\ucon ) \right) 
    &= f( \xvec(t+\tau), \ucon ) .
    \label{eq:koopman-applied}
\end{align}
for a constant input $\ucon$ over the time interval $[t,t+\tau]$.

The set of Koopman operators is generated by an infinitesimal generator, denoted $\koop$, according to the following relation \Dan{cite}
\begin{align}
    \koop_\tau &= e^{\tau \koop}
    \label{eq:generator}
\end{align}
The infinitesimal generator describes the time derivative of observables along trajectories of the system
\begin{align}
    \koop f &= \frac{d}{dt} f
\end{align}
such that
\begin{align}
    ( \koop f ) (\xvec(t) , \uvec(t)) &= \frac{\partial f}{\partial \xvec} \Fvec (\xvec(t) , \uvec(t) )
    \label{eq:generator-applied}
\end{align}
For a given time-step, $\koop_\tau$ is sometimes referred to as the \emph{discrete time} Koopman operator and $\koop$ as the \emph{continuous time} Koopman operator \Dan{cite}.

%% Introduce the idea of basis
Let $\{\psi_i\}$ be a basis for the space of observables $\mathcal{F}$.
Any observable $f$ can be represented as a linear combination of the basis functions
\begin{align}
    f &= \theta_1 \psi_1 + \theta_2 \psi_2 + \cdots
\end{align}
And the effect of the Koopman operator acting on an observable can be represented by a set of coefficients $\{ k_{i} \}_{i=1}^N$
\begin{align}
    \frac{d}{dt} f &= \koop f = \sum_{i=1}^N k_{i} \psi_i
\end{align}
So if we choose a set of observables and stack them together into a vector
\begin{align}
    \frac{d}{dt}
    \begin{bmatrix} {\psi}_1 \\ {\psi}_2 \\ \vdots \end{bmatrix}
    &=
    \begin{bmatrix} \koop \psi_1 \\ \koop \psi_2 \\ \vdots \end{bmatrix}
    =
    \begin{bmatrix} k_{11} \psi_1 + k_{12} \psi_2 + k_{13} \psi_3 + \cdots \\
    k_{21} \psi_1 + k_{22} \psi_2 + k_{23} \psi_3 + \cdots \\
    \vdots \end{bmatrix}
\end{align}


%% How to get the dynamics of the state
Since this is true for \emph{any} observable function $f$, the Koopman operator can be used to describe the evolution of the state itself by applying it to the set of indicator functions $\{ f_i : f_i (\xvec(t) , \uvec(t)) = x_i (t) \}_{i=1}^n$ where $x_i(t)$ represents the $i^\text{th}$ component of the vector $\xvec(t)$ and stacking the results as a vector:
\begin{align}
    \xvec( t + \tau ) 
    = \begin{bmatrix} \mathcal{K}_{\tau} f_1 \left( \xvec (t) , \uvec(t) \right) \\ \vdots \\ \mathcal{K}_{\tau} f_n \left( \xvec (t) , \uvec(t) \right) \end{bmatrix}
    \label{eq:xstep} 
    && \text{or} \hspace{12pt}
    \dot{\xvec}( t ) 
    = \begin{bmatrix} \koop f_1 \left( \xvec (t) , \uvec(t) \right) \\ \vdots \\ \koop f_n \left( \xvec (t) , \uvec(t) \right) \end{bmatrix}.
    \label{eq:xdot}
\end{align}
In this way, the Koopman operator provides an infinite-dimensional linear representation of a nonlinear dynamical system \cite{budivsic2012applied}.
%% Sometimes we want to define K on just a subspace
It is sometimes possible to restrict the Koopman operator to a subspace $\bar{\mathcal{F}}$ of the space of all observable functions.
This is only possible if all functions in the subspace remain in the subspace after being acted on by the Koopman operator.
This type of subspace is called a Koopman invariant subspace...

%% Def: Koopman invariant subspace
\begin{definition}[Koopman invariant subspace \Dan{rough draft}]
A subspace $\bar{\mathcal{F}} \subset \mathcal{F}$ is said to be Koopman invariant if the action of the (continuous) Koopman operator doesn't leave the subspace, i.e.
\begin{align}
    \koop f &\in \bar{\mathcal{F}}
    && \forall f \in \bar{\mathcal{F}}
    \label{eq:kis}
\end{align}
\label{def:koopman-invariant-subspace}
\end{definition}

%% Thm: Koopman invariant subspace with a specific basis
\begin{theorem}
\Dan{rough draft, maybe not separate theorem because obvious from definition}
Let $\{ \psi_i \}_{i=1}^{\infty}$ \Dan{could be finite} be a basis for the subspace $\bar{\mathcal{F}} \subset \mathcal{F}$. If $\bar{\mathcal{F}}$ is Koopman invariant with respect to the dynamical system \eqref{eq:nlsys}, then the following condition holds for all $i$:
\begin{align}
    % \frac{d}{dt} \psi_i &= 
    \frac{\partial \psi_i}{\partial x} F \in \text{span}( \psi_i )
    \label{eq:span-psi}
\end{align}
\label{thm:span-kis}
\end{theorem}
\begin{proof}
This is verified by applying the Koopman operator to an arbitrary basis function $\psi_i$:
\begin{align}
    \koop \psi_i &\in \bar{\mathcal{F}} && \text{By Def. } \eqref{def:koopman-invariant-subspace} \\
    \frac{d}{dt} \psi_i &\in \text{span}( \psi_i ) && \text{By } \eqref{eq:generator} \\
    \frac{\partial \psi_i}{\partial x} F &\in  \text{span}( \psi_i )   && \text{By } \eqref{eq:generator-applied}
\end{align}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Model realizations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model realizations} \label{sec:realizations}

Given an input signal $u(t)$ and corresponding state response $x(t)$, a realization is a dynamical system model that generates the same output for given inputs

\Dan{Define linear, bilinear, and nonlinear realizations in terms of a (possibly) infinite dimensional variable z.}

%% Realization
\begin{definition}[Realization]
A realization of a dynamical system is a dynamical system that generates identical input-output behavior.
For in input $\uvec$, output $\xvec$, and state $\zvec$, a realization is linear if for some $\alpha,\beta$ ...
\begin{align}
    \frac{d}{dt} \zvec(t) &= G( \zvec(t) , \uvec(t) ) \\
    \yvec(t) &= C( \zvec(t) )
\end{align}
\label{def:realization}
\end{definition}

%% Linear realization
\begin{definition}[Linear realization]
\Dan{As written this definition is specific to a specific context, not general.}
A linear realization of a system \eqref{eq:nlsys} is a set of observables $\{ z_i \in \mathcal{X} \}_{i=1}^N$ such that for every $i$,
\begin{align}
    \dot{z}_i &= \sum_{j=1}^N \alpha_j z_j + \sum_{j=1}^m \beta_j u_j \\
    % z_i &\in \mathcal{X} 
    % &= \text{func}(\xvec)
\end{align}
for some $\{ \alpha \} \in \Real$ and $\{ \beta \} \in \Real$.
\label{def:linear-realization}
\end{definition}

%% Bilinear realization
\begin{definition}[Bilinear realization]
\begin{align}
    \dot{z}_i &= \sum_{j=1}^N \alpha_j z_j + \sum_{j=1}^m \beta_j u_j + \sum_{j=1}^N \sum_{k=1}^m h_{jk} z_j u_k \\
    z_i &\in \mathcal{X}
    % z_i &= \text{func}(\xvec)
\end{align}
\label{def:bilinear-realization}
\end{definition}

%% Nonlinear realization
\begin{definition}[Nonlinear realization]
\begin{align}
    \dot{z}_i &= \sum_{j=1}^N \alpha_j z_j \\
    z_i &\in \mathcal{F}
    % z_i &= \text{func}( \xvec , \uvec )
\end{align}
\label{def:nonlinear-realization}
\end{definition}

%% Koopman operator flows dynamics forward, but not in format we can use
The Koopman operator describes the evolution of the values of observable along trajectories of a dynamical system, but does not directly describe the evolution of the system itself.
To do that, we need to choose a set of observables to act as our ``lifted state'' in the space of observables, (and define a projectiong from the lifted state to the original state)

Define a subspace of $\mathcal{F}$ by choosing a set of basis functions.

Depending on the subspace/basis functions, different types of realizations will be possible.

Describe different types of realizations (make it generic so it can admit infinite dimensional realizations)


This section describes how to utilize a matrix approximation of the Koopman operator to construct model realizations that describe the input-output behavior of a system.

% \input{theorems/thm_realization-n&s-conditions}
% \input{theorems/thm_bilinear}
% \input{theorems/thm_scratch}
\input{theorems/thm_in-span}
\input{theorems/realizations}







% We specify these conditions in terms of the concept of Koopman invariant subspaces, defined in \Dan{cite Brunton} as follows:

% %% Def: Koopman invariant subspace
% \begin{definition}[Koopman invariant subspace]
% \Dan{Don't need this def. anymore} A subspace $\bar{\mathcal{F}} \subset \mathcal{F}$ is said to be Koopman invariant if all observables $f$ in the subspace remain in the subspace after being acted on by the Koopman operator, i.e.
% \begin{align}
%     \koop f &\in \bar{\mathcal{F}}
%     && \forall f \in \bar{\mathcal{F}}
%     \label{eq:kis}
% \end{align}
% \label{def:koopman-invariant-subspace}
% \end{definition}

% With this definition in hand, we can describe the conditions that must be satisfied in order for a chosen set of observables to admit a linear and/or bilinear realization.

==> unused/intro_unused_text.tex <==
%
A valid Koopman representation, however, is 
Koopman models with bilinear control inputs, i.e. functions that are linear with respect to the control input when the state is fixed
While system models with linear control inputs are desirable because of their computational efficiency and compatibility with linear control techniques, models with bilinear control inputs preserve some of the computational benefits of linear models without
An alternative to models with linear control inputs is


%% Conditions for linear Koopman model are difficult to satisfy
In this paper, we present necessary and sufficient conditions for a given nonlinear dynamical system [with control inputs] to have a valid Koopman representation in a subspace spanned by a chosen set of observables.
Despite the demonstrated success of Koopman approximations with linear inputs in predicting the behavior of some systems,
we show that the conditions under which a valid Koopman representation exists are exceedingly difficult to satisfy for a set of observables that contains only linear functions of the input.
% without up front knowledge of the underlying dynamics of a system.
% Therefore, for unknown controlled dynamical systems, linear Koopman representations will often come up short
However, the conditions are much easier to satisfy for a set of observables that contains both linear and bilinear functions of the input.
% However, the conditions under which a valid bilinear Koopman representation exists are much less restrictive.

For a particular subspace of observables, there is no guarantee that the Koopman operator restricted to that space
If the dynamics of a system are completely unknown, there is no guarantee that a
valid Koopman 
finite-dimensional approximation of the Koopman operator will accurately describe the system.
But, if the approximation is identified on a set of observables
in a particular subspace of obervables will  

This implies that, if the dynamics of a system are unknown, a Koopman approximation with bilinear inputs is more likely 

%% Benefits of bilinear realizations
This property is of the utmost importance when the dynamics of a system are unknown


%%

This fact regarding the convergence of Koopman representations is especially inconvenient in the context of system identification of unknown dynamics.
In such cases, if it 



%% 
This paper presents necessary and sufficient conditions for a given nonlinear dynamical system with control inputs to have a valid Koopman representation in a specified subspace of observables.


If the underlying dynamics of a system are known, 

presents some real challenges for system identification of unknown systems




%% 
In this paper, we argue that











%% 
In practice, we enforce that the Koopman representation be linear with respect to the control input by restricting it to a subspace of observables that does not include nonlinear functions of the input. 


%% In practice, 
For a given dynamical system, there may be a finite dimensional Koopman repres...
Thus, when using Koopman representations of nonlinear systems, one must consider both  there are two major considerations

Approximations of the Koopman operator have been identified from data then used to control nonlinear dynamicl systems using linear control methods.

%% Focus of this paper
This paper 


%% We force it to be linear by choosing basis functions a certain way
To ensure that a Koopman representation is linear with respect to the control input, we must restrict it to a specific subspace of observables.
As we will see, not all nonlinear dynamical systems have an equivalent Koopman representation in this subspace

%% How a Koopman operator is identified on a subspace
Finite-dimensional representations are identified by restricting the Koopman operator to a subspace spanned by a chosen set of scalar-valued functions.
Within such a subspace, the Koopman operator can be constructed from data using a technique called Extended Dynamic Mode Decomposition \Dan{cite}, or via the Koopman Canonical Transform (KCT) if its eigenfunctions are known \Dan{cite Goswami}.

%% But the choice of basis functions/subspace determines if a realization is possible


%% Prior work using Koopman linearizations
In Korda/Mezic, truncated representations of the Koopman operator are constructed
Truncated representations of the Koopman operator can be constructed from data \Dan{cite}, eigenfunctions \Dan{cite}, or ---

%% How the Koopman operator gives you global linearization
Koopman operator theory provides the theoretical foundation/underpinnings for global linearization



==> unused/realizations.tex <==
\begin{theorem}[] \label{thm:realizations}

Let $\bar{\mathcal{Z}} \subset \mathcal{Z}$ be the span of the set of observables $\{ z_i \in \mathcal{Z} \}_{i=1}^N$.
The realization over this set is:
\begin{enumerate}
    \item \textbf{Linear} if an only if
    $\bar{\mathcal{Z}} \cup \mathcal{U}$ is a Koopman invariant subspace and $\mathcal{X} \subset \bar{\mathcal{Z}}$.
    \item \textbf{Bilinear} if and only if $\bar{\mathcal{Z}} \cup \mathcal{U} \cup \{ f \cdot g \vert f \in \bar{\mathcal{Z}} , g \in \mathcal{U} \}$ is a Koopman invariant subspace and $\mathcal{X} \subset \bar{\mathcal{Z}}$ \Dan{only if}.
\end{enumerate}
Note that linear systems are by definition also bilinear.
\Dan{This version of theorem is compatible with discrete systems, I may rewrite everything in terms of discrete systems.}
\end{theorem}

\begin{proof}
\Dan{Rough draft in notebook, to be inserted later}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/proof-realization.jpg}
    \label{fig:proof}
\end{figure}
\end{proof}

==> unused/thm_bilinear.tex <==
\begin{theorem}[] \label{thm:bilinear}
% Necessary and sufficient conditions for linear realization

Given a (possibly infinite) set of observables ${\{ \psi_i : \Real^n \to \Real \}_{i=1}^N}$,
the (nonlinear) dynamical system
\begin{align}
    \dot{\xvec} &= F_x (\xvec) + F_{xu} (\xvec,\uvec)
\end{align}
% where $\xvec \in X \subset \Real^n$ and $\uvec \in U \subset \Real^m$,
has a bilinear realization in the space spanned by the observables
% \begin{align}
%     \dot{\zvec} &= A \zvec + B \uvec
% \end{align}
% \begin{align}
%     \frac{d}{dt} \begin{bmatrix} \psi_1(\xvec) \\ \psi_2(\xvec) \\ \vdots \end{bmatrix} &=
%         \begin{bmatrix} a_{11} & a_{12} & \cdots \\ a_{21} & a_{22} & \cdots \\ \vdots & \vdots & \ddots \end{bmatrix}
%         \begin{bmatrix} \psi_1(\xvec) \\ \psi_2(\xvec) \\ \vdots \end{bmatrix} +
%         \begin{bmatrix} b_{11} & \cdots & b_{1m} \\ b_{21} & \cdots & b_{2m} \\ \vdots & \vdots & \vdots \end{bmatrix} \uvec
% \end{align}
% \begin{align}
%     \frac{d\psivec}{dt} (\xvec) &=
%         \begin{bmatrix} a_{11} & a_{12} & \cdots \\ a_{21} & a_{22} & \cdots \\ \vdots & \vdots & \ddots \end{bmatrix}
%         \psivec(\xvec) +
%         \begin{bmatrix} b_{11} & \cdots & b_{1m} \\ b_{21} & \cdots & b_{2m} \\ \vdots & \vdots & \vdots \end{bmatrix} \uvec
% \end{align}
if and only if for every observable $\psi_i$ there exists sets of coefficients $\{ a_{ij} \}_{j=1}^N$, $\{ b_{ij} \}_{j=1}^m$, and $\{ h_{ijk} \}_{j,k=1}^N$ such that the following conditions hold $\forall \xvec \in X, \uvec \in U$:
\begin{align}
    \frac{\partial \psi_i}{\partial \xvec} F_x(\xvec) &= \sum_{j=1}^N a_{ij} \psi_j(\xvec) \\
    \frac{\partial \psi_i}{\partial \xvec} F_{xu}(\xvec,\uvec) &= \sum_{j=1}^m \left( b_{ij} + \sum_{k=1}^N h_{ijk} \psi_k(\xvec) \right) u_j
\end{align}

\end{theorem}

==> unused/thm_in-span.tex <==
\begin{theorem}[] \label{thm:in-span}

\Dan{This is just a quick draft not final theorem.}
The (nonlinear) dynamical system admits a linear realization if there exists a set of basis functions of the form
\begin{align}
    \psi_i(\ycon,\ucon) &=
    \begin{cases}
        g_i(\ycon), \quad \forall i \in \{1,\ldots, N-m\}  \label{eq:gi} \\
        \ucon_{i-(N-m)}, \quad \forall i \in \{N-m+1, \ldots, N\} \label{eq:ui}
    \end{cases}
    \label{eq:basis-linear}
\end{align}

such that for each basis function 
\begin{align}
    \frac{\partial \psi_i}{\partial x} F \in \text{span of } \{ \psi_i \}_{i=1}^N
\end{align}

It has a bilinear realization if there exists a set of basis functions of the form
\begin{align}
    \psi_i ( \ycon , \ucon ) &= 
    \begin{cases}
        g_i (\ycon) & i \in \{ 1 , ... , N \} \\
        g_{i-N} (\ycon) \, \tilde{u}_1 & i \in \{ N+1 , ... , 2N \} \\
        & \vdots \\
        g_{i-Nm} (\ycon) \, \tilde{u}_m & i \in \{ Nm+1 , ... , N(m+1) \} \\
        \ucon_{i - N(m+1)} & i \in \{ N(m+1)+1 , ... , N(m+1)+m \}
    \end{cases}
    \label{eq:basis-bilinear}
\end{align}

such that for each basis function 
\begin{align}
    \frac{\partial \psi_i}{\partial x} F \in \text{span of } \{ \psi_i \}_{i=1}^N
\end{align}

\end{theorem}





%% What it takes to be a valid realization in the first place
\begin{theorem}[] \label{thm:in-span}
\Dan{Quick draft of theorem}

The subspace spanned by a set of basis functions admits a valid/consistent realization/representation of the the (nonlinear) dynamical system with respect to the lifted state $\psivec(\xvec,\uvec)$ if and only if for every $\psi_i$ (basis function)
\begin{align}
    \frac{\partial \psi_i}{\partial x} F \in \text{span of } \{ \psi_i \}_{i=1}^N
\end{align}

If a set of basis functions of this form --(linear basis)-- admits a valid realization, then that realization is linear.

If a set of basis functions of this form --(bilinear basis)-- admits a valid realization, then that realization is bilinear.
\end{theorem}
\begin{proof}

\Dan{Can't do this because you are trying to prove that the generator exists in the first place.}
Apply the definition of the Koopman generator to each basis function.
A linear operator applied to a basis function has to give you a linear combination of the basis functions back (those are the columns of the matrix).
\end{proof}


A subspace admits a linear representation if and only if it is spanned by basis functions of the following form --(linear basis functions)-- and admits a valid realization.

==> unused/thm_realization-n_s-conditions.tex <==
\begin{theorem}[] \label{thm:n-and-s-conditions}
% Necessary and sufficient conditions for linear realization

Given a (possibly infinite) set of observables ${\{ \psi_i : \Real^n \to \Real \}_{i=1}^N}$,
the (nonlinear) dynamical system
\begin{align}
    \dot{\xvec} &= F_x (\xvec) + F_{xu} (\xvec,\uvec)
\end{align}
% where $\xvec \in X \subset \Real^n$ and $\uvec \in U \subset \Real^m$,
has a linear realization in the space spanned by the observables
% \begin{align}
%     \dot{\zvec} &= A \zvec + B \uvec
% \end{align}
% \begin{align}
%     \frac{d}{dt} \begin{bmatrix} \psi_1(\xvec) \\ \psi_2(\xvec) \\ \vdots \end{bmatrix} &=
%         \begin{bmatrix} a_{11} & a_{12} & \cdots \\ a_{21} & a_{22} & \cdots \\ \vdots & \vdots & \ddots \end{bmatrix}
%         \begin{bmatrix} \psi_1(\xvec) \\ \psi_2(\xvec) \\ \vdots \end{bmatrix} +
%         \begin{bmatrix} b_{11} & \cdots & b_{1m} \\ b_{21} & \cdots & b_{2m} \\ \vdots & \vdots & \vdots \end{bmatrix} \uvec
% \end{align}
% \begin{align}
%     \frac{d\psivec}{dt} (\xvec) &=
%         \begin{bmatrix} a_{11} & a_{12} & \cdots \\ a_{21} & a_{22} & \cdots \\ \vdots & \vdots & \ddots \end{bmatrix}
%         \psivec(\xvec) +
%         \begin{bmatrix} b_{11} & \cdots & b_{1m} \\ b_{21} & \cdots & b_{2m} \\ \vdots & \vdots & \vdots \end{bmatrix} \uvec
% \end{align}
if and only if for every observable $\psi_i$ there exists sets of coefficients $\{ a_{ij} \}_{j=1}^N$ and $\{ b_{ij} \}_{j=1}^m$ such that the following conditions hold $\forall \xvec \in X, \uvec \in U$:
\begin{align}
    \frac{\partial \psi_i(\xvec)}{\partial \xvec} F_x(\xvec) &= \sum_{j=1}^N a_{ij} \psi_j(\xvec) \\
    \frac{\partial \psi_i(\xvec)}{\partial \xvec} F_{xu}(\xvec,\uvec) &= \sum_{j=1}^m b_{ij} u_j
\end{align}

\end{theorem}

==> unused/thm_scratch.tex <==
\begin{theorem}[] \label{thm:bilinear}
% Necessary and sufficient conditions for linear realization

Given a (possibly infinite-dimensional) vector valued observable ${ \psivec : \Real^n \to \Real^N }$,
the (nonlinear) dynamical system
\begin{align}
    \dot{\xvec} &= F_x (\xvec) + F_{xu} (\xvec,\uvec)
\end{align}
% where $\xvec \in X \subset \Real^n$ and $\uvec \in U \subset \Real^m$,
has a bilinear realization with respect to the observable
% \begin{align}
%     \dot{\zvec} &= A \zvec + B \uvec
% \end{align}
% \begin{align}
%     \frac{d}{dt} \begin{bmatrix} \psi_1(\xvec) \\ \psi_2(\xvec) \\ \vdots \end{bmatrix} &=
%         \begin{bmatrix} a_{11} & a_{12} & \cdots \\ a_{21} & a_{22} & \cdots \\ \vdots & \vdots & \ddots \end{bmatrix}
%         \begin{bmatrix} \psi_1(\xvec) \\ \psi_2(\xvec) \\ \vdots \end{bmatrix} +
%         \begin{bmatrix} b_{11} & \cdots & b_{1m} \\ b_{21} & \cdots & b_{2m} \\ \vdots & \vdots & \vdots \end{bmatrix} \uvec
% \end{align}
% \begin{align}
%     \frac{d\psivec}{dt} (\xvec) &=
%         \begin{bmatrix} a_{11} & a_{12} & \cdots \\ a_{21} & a_{22} & \cdots \\ \vdots & \vdots & \ddots \end{bmatrix}
%         \psivec(\xvec) +
%         \begin{bmatrix} b_{11} & \cdots & b_{1m} \\ b_{21} & \cdots & b_{2m} \\ \vdots & \vdots & \vdots \end{bmatrix} \uvec
% \end{align}
if and only if there exists $A \in \Real^{N \times N}$, $B \in \Real^{N \times m}$, and $\{ H_j \in \Real^{N \times N} \}_{j=1}^m$ such that the following conditions hold $\forall \xvec \in X, \uvec \in U$:
\begin{align}
    \frac{\partial \psivec}{\partial \xvec} F_x(\xvec) &= A \psi\vec(\xvec) \\
    \frac{\partial \psivec}{\partial \xvec} F_{xu}(\xvec,\uvec) &= B \uvec + \sum_{j=1}^m H_j \psivec(\xvec) u_j
\end{align}

\end{theorem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DEFINITIONS: OLD VERSIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Linear realization
\begin{definition}[Linear model realization]
A model realization defined over the set of observables $\{ z_i \in \mathcal{Z} \}_{i=1}^N$ is linear if there exist sets of coefficients ${ \{ \alpha_{ij} \in \Real \}_{i=1,j=1}^{N,N} }$, ${ \{ \beta_{ij} \in \Real \}_{i=1,j=1}^{N,m} }$, and ${ \{ c_{ij} \in \Real \}_{i=1,j=1}^{n,N} }$ such that
\begin{align}
    \frac{d}{dt} z_i &= \sum_{j=1}^N \alpha_{ij} z_j + \sum_{j=1}^m \beta_{ij} u_j && \text{for } i = 1,\ldots,N \\
    x_i (t) &= \sum_{j=1}^N c_{ij} z_j(t) && \text{for } i = 1,\ldots,n
\end{align}
\label{def:linear-realization}
\end{definition}

%% Bilinear realization
\begin{definition}[Bilinear model realization]
A model realization defined over the set of observables ${ \{ z_i \in \mathcal{Z} \}_{i=1}^N }$ is bilinear if there exist sets of coefficients 
${ \{ \alpha_{ij} \in \Real \}_{i=1,j=1}^{N,N} }$, 
${ \{ \beta_{ij} \in \Real \}_{i=1,j=1}^{N,m} }$, 
${ \{ h_{ijk} \in \Real \}_{i=1,j=1,k=1}^{N,N,m} }$, 
and ${ \{ c_{ij} \in \Real \}_{i=1,j=1}^{n,N} }$
such that
\begin{align}
    \frac{d}{dt} z_i &= \sum_{j=1}^N \alpha_{ij} z_j + \sum_{j=1}^m \beta_{ij} u_j + \sum_{j=1}^N \sum_{k=1}^m h_{ijk} z_{j} u_{k}
    % && \text{for } i = 1,\ldots,N
\end{align}
for $i = 1 , \ldots , N$ and
\begin{align}
    x_i (t) &= \sum_{j=1}^N c_{ij} z_j(t)
    % && \text{for } i = 1,\ldots,n
\end{align}
for $i = 1 , \ldots , n$.
\label{def:bilinear-realization}
\end{definition}
